StackSight: Unveiling WebAssembly through Large Language Models and Neurosymbolic Chain-of-Thought Decompilation

WebAssembly enables near-native execution in web applications and is increasingly adopted for tasks that demand high performance and robust security. However, its assembly-like syntax, implicit stack machine, and low-level data types make it extremely difficult for human developers to understand, spurring the need for effective WebAssembly reverse engineering techniques. In this paper, we propose StackSight, a novel neurosymbolic approach that combines Large Language Models (LLMs) with advanced program analysis to decompile complex WebAssembly code into readable C++ snippets. StackSight visualizes and tracks virtual stack alterations via a static analysis algorithm and then applies chain-of-thought prompting to harness LLM's complex reasoning capabilities. Evaluation results show that StackSight significantly improves WebAssembly decompilation. Our user study also demonstrates that code snippets generated by StackSight have significantly higher win rates and enable a better grasp of code semantics.

==> tex/baselines.tex <==
\subsection{Baselines}

\subsubsection{In-Context Learning}

A baseline approach is to elicit LLM's In-Context Learning (ICL) ability ~\cite{dai2023gpt} by providing it with one or more examples as context. It is also known as zero-shot or few-shot learning, which involves presenting Large Language Models (LLMs) with zero or a small number of examples to provide context and understanding of a specific task. Such a method is widely applied for its simplicity and ability to quickly adapt to new tasks without the need of training or fine-tuning. 

However, our experiments reveal that In-Context Learning faces challenges in the reverse engineering tasks such as WebAssembly decompilation. Without the intermediate steps, it is hard for LLM to logically bridge the low-level WebAssembly code and the corresponding expected C/C++ code. This finding underscores the complexity of such decompilation tasks and the need for more specialized approaches. We include ICL as a comparative baseline in our evaluation. The comparison serves to demonstrate the superiority of our approach in breaking the task down to a series of subtasks, thus accurately translating and preserving the functionality of WebAssembly code in its high-level C/C++ code representation. We conduct ICL baselines on gpt-3.5-turbo-1106~\footnote{\url{https://platform.openai.com/docs/models/gpt-3-5}} and Code Llama~\cite{rozière2023code}.

\noindent \textbf{In-Context Learning Prompt Construction}
We construct in-context learning examples by concatenating three parts. We first start with an instruction part to explicitly state that the task to perform is to decompile WebAssembly files into the corresponding C++ file. We then append one round of user and AI system interaction to serve as in-context learning example. The user input is the \texttt{.wat} file, while the exemplar system output is the corresponding C++ file used to compile. Finally, we append the target \texttt{.wat} file of interest. For an example prompt, please refer to Appendix \ref{in_context_prompt_eg}



% \textcolor{blue}{The following are works to improve the pipeline with more context, which we may or may not do in this paper}

% In our methodology, we leverage LLM's In Context Learning (ICL) ability~\cite{dai2023gpt} to enhance the performance of our decompilation pipeline. We contextualize the pipeline by 1). Providing a knowledge base for wasm syntax and decompilation rules, and 2). Providing a representative decompilation pattern to standardize and supplement the ICL process. 

% In particular, it has been shown that by providing LLMs with input patterns alongside tokens, the correctness and determinism of the output tokens are drastically increased~\cite{LIU2023,brown2020language}. In our pipeline, we utilize this fine-tuning capability of LLM and establish a systematic format of decompilation steps. Since the objective of engaging ICL is to remove non-determinism in the decompilation pipeline, the complexity and heuristic of the chosen example are trivial.



==> tex/intuition.tex <==
\subsection{Intuition on Step-By-Step Decompilation}
Motivated by the step-by-step problem-solving paradigm, we reflect on how humans would approach the WebAssembly decompilation task step-by-step. For human developers, we identify the following \textbf{three} intuitions that are critical to unveil the assembly-like nature of WebAssembly code.


\noindent \textbf{Explicitly Tracking the Virtual Stack}\quad As specified in the original paper~\cite{webassembly}, WebAssembly code operates on an implicit stack. An example WebAssembly Text Format file is as follows.

\begin{lstlisting}[style=customwat, label={lst:wat}]
(module
(type (;0;) (func))
(type (;1;) (func (param i32) (result i32)))
(func (;0;) (type 0))
(func (;1;) (type 1) (param i32) (result i32)
    local.get 0
    i32.const 1
    i32.add
    local.get 0
    i32.mul
    i32.const 2
    i32.div_s)
(export "__wasm_call_ctors" (func 0))
(export "__wasm_apply_data_relocs" (func 0))
(export "_Z8sum_to_ni" (func 1)))
\end{lstlisting}

As show in this snippet, WebAssembly code loads variables onto the stack (\lstinline[style=customwat]{local.get, i32.const}), operates on the top elements on the stack and writes back the answer (\lstinline[style=customwat]{i32.add, i32.mul, i32.div_s}). However, there is no representation in the text format file that explicitly tracks the history states of the stack.

While this approach can achieve a more compact code size, it also imposes great difficulties for humans to understand the code. We concur that keeping an explicit history of what is on the virtual stack and the operations that interact with the stack would serve as a useful intermediate step. More than helping to identify the semantics of WebAssembly code, this step also reveals patterns in \texttt{.wat} files that correspond to specific behavior in C++ source code. 
By making variable computations and relationships explicit, we emulate the logical process a developer would use when confronting WebAssembly code. Specifically, our static analysis algorithm annotates each code line with the current virtual stack state, noting variable assignments and control flow statements, such as 'break' or 'continue' in loops.  
This explicit representation of variable relationships sets the stage for the next step: revealing the semantic purposes of each variable.

\noindent \textbf{Recovering Semantically Meaningful Names of Variables}\quad Also specified in the original paper~\cite{webassembly}, WebAssembly code only assigns an index to used variables. This is another major obstacle in understanding WebAssembly code. For human developers, we encode a large amount of semantic information in the name of variables. To recover variable semantics of WebAssembly code, we first prompt the LLM to predict the variable types of input and return values based on the stack information. Then, the model can gradually identify the purpose of each local variable by looking at computational relationship of each local variable. 
%Therefore, we also agree on recovering semantically meaningful names for used variables. 
%This intuition is also supported by our discovery that the WebAssembly compiler follows certain conventions when assigning local variables. One type of information tends to be stored at a specific index.

\noindent \textbf{Summarize in Natural Language}\quad Once all variable semantics are recovered, the next logical step for human developers to interpret the WebAssembly code is to identify high-level purposes of the code. 
This is crucial in preventing the verbatim transcription of WebAssembly instructions into potentially incorrect C/C++ code. Our approach focuses on a natural language interpretation of each part of the code, which provides a more intuitive understanding of the code's functionality, aligning with how developers typically conceptualize complex coding structures.


\subsection{Pipeline}
\begin{figure*}[h]
    \centering
    % \vspace{-0.5em}
    \includegraphics[width=1.9\columnwidth]{figs/pipeline_v3.pdf}
    \caption{The decompilation pipeline.}
    \label{fig:pipeline}
    %\vspace{-1em}
\end{figure*}

To facilitate stepwise reasoning, we build a pipeline shown in Figure~\ref{fig:pipeline} for WebAssembly decompilation, where each component focuses on one of the above decompilation phase. This structured pipeline ensures that it can progressively build upon its understanding, mirroring how a human will make sense of and decompile a piece of WebAssembly code. It works as follows:

Given a piece of binary WebAssembly code (\texttt{.wasm}), we first translate it to the WebAssembly text format (\texttt{.wat}) using \texttt{wasm2wat} tool in WebAssembly Binary Toolkit (WABT)~\footnote{https://github.com/WebAssembly/wabt}. Then we design a static analysis algorithm to annotate each line of code with the current state of the stack and notes for variable assignment and control flow arguments. Our goal is to make the virtual stack machine in WebAssembly explicit, translating implicit stack operations into more transparent constructs for the model to understand such low-level operations. As WebAssembly has a finite set of operations or opcodes and each opcode has specific rules on how it manipulates the stack, a static analysis approach is chosen over a machine learning approach. 
Our algorithm is transparent and deterministic: Given an instruction and the current state of the stack, the resulting stack is precisely determined. It supports the visualization of stack for all 172 WebAssembly Opcodes, multiple function calls, control flow and branching statements.


The annotated WebAssembly code (\texttt{.wat}) is then included in the prompt to a large language model in a step-by-step manner. First, based on the stack visualization, we ask the LLM to comprehend variable relationships, predict the data types for input parameters and return types (\textit{pivot variables}), and attempt to recover the semantic meaning of each local variable based on the pivot variables. Then, given the context and usage of each local variable, the model is asked to summarize the function operations in natural language to derive a high-level understanding of what the WebAssembly code is doing. Finally, based on the above steps, the LLM is prompted to decompile the piece of WebAssembly code to C or C++. To evaluate the outputs from the LLM, we design a test oracle that incorporates a series of test cases to evaluate the correctness of the decompiled code. 
%Compilation errors and failed test cases are passed as feedback to the prompt generator to prompt the model for another round of generation. Such iterative process will improve the generation over time, and will terminate if the pass rate goes above a certain threshold or the number of iterations exceed the query budget. \textcolor{red}{Due to the nondeterministic nature of LLM such as GPT, we would ideally repeat each prompt for a number of times to get a more diverse set of outputs. Our robustness study in Section \ref{sec:robustness} shows that predictions are rather stable given the same query and seed. In practice, we employ the threshold of pass rate to be xx.}
